Modeling and optimal control of growth, energy, and resource dynamics of Hermetia illucens in mass production environment

Mass production of Hermetia illucens insect larvae is now being adopted in many countries and is taking an industrial production approach. Despite abundant literature on factors that affect larvae growth and the optimal static parameters identified in laboratory setup, for an industrial production process it is necessary to identify the trajectories such that the growth as well as the production process is optimal. To achieve this in this work, some of the important requirements and challenges involved thereof are identified and objectives of the automation process are formulated within a model based optimal control setup. Mechanistic models necessary for the optimization framework are derived as differential equations that describe the dynamic variation of resources (feed, water, O2 etc.), energy, and larval biomass. In addition, the elevated metabolic activity of larvae corresponding to the final instar development is identified and also modelled based on the observation from experiments. The mass and energy balance approach used in modelling enables the quantification and distinction of the mass and energy flux components in various levels (e.g. larvae body, growing medium, production environment, and external environment) while holding its applicability for both open and closed/reactor based production setups. Finally, the trajectories generated using the synthesized optimal controller are tested under different scenarios showcasing significant reduction in resource consumption compared to a fixed set-point operation of the production setup. Results presented in this work not only showcase the potential of the mechanistic models and their application in identifying the relevant process parameters (e.g. reactor properties such as volume, thermal conductivity, actuator capacities), but most importantly in optimizing the process dynamically and tuning the process objectives as desired.

==> 02_experiment_description.tex <==
\subsection{Experiments}
%\red{Include list of parameters that is logged for all experiments}
Young larvae and feed were obtained from Hermetia Baruth GmbH. 
%(\textcolor{blue}{The substrate consist of a mixture of \textcolor{red}{10\%} malt seed, \textcolor{red}{20 \%} colza meal, \textcolor{red}{60 \%} triticale and \textcolor{red}{10 \%} wheat flour} OR \textcolor{blue}{one part wheat bran dry matter and three parts pig feed} \textcolor{purple}{In my old document the first (detailed) part was commented out and the second part was left; I am not sure why I did that, it might have been so Hermetia doesn't bother us because we published their 'secret' recipe?}) were obtained from Hermetia Baruth GmbH.
Dry feed consists of one part wheat bran dry matter and three parts pig feed.
Substrate is prepared by mixing one part dry feed and three parts water.
Neonates at Hermetia Baruth GmbH were raised on the same feed used in the experiments.
After measuring larval fresh weight, larvae are subjected to -10\si{\celsius} in a freezer for at least 24~\si{\hour}.
Afterwards they are dried for 6~\si{\hour} at 70\si{\celsius} in an air dryer.

\paragraph{Influence of temperature on growth}
The experiments were performed to evaluate the influence of temperature on larval growth.
Three stainless steel trays were filled with 2.0~\si{\kilogram} of substrate to achieve a substrate depth of about 3-5~\si{\centi\meter}. 
2000 larvae of about 10 days old with a mean weight of \SI{4.28}{\milli\gram} were then introduced into each steel tray.
The trays were then placed in three different growing chambers.
The air temperature inside the the three growing chambers were set to 25~\si{\celsius}, 29~\si{\celsius} and 33~\si{\celsius} respectively.
Larval weight and weight of the whole tray was measured daily after the second day of the experiment.
From fourth day onwards, larvae samples were dried and dry weight measurement were made.
Growing chambers were mostly closed, air was ventilated through the air pump in a 10~\si{\minute} ON and 20~\si{\minute} OFF cycles.
Due to the this ventilation strategy and a relatively large substrate surface area, humidity was at~$>90\%$.
Growing chambers were only opened to obtain samples of larvae for measurements.
Nine samples were collected over the course of twelve days.
Sample sizes ranged from 50 to 87.
The data sets are referred to as TG1-TG3.
The raw data obtained in the experiment TG2 (temperature set point of \SI{30}{\celsius}) can be seen in the figure \ref{fig:T_experiments_data}.

% \paragraph{Substrate evaporation (\red{can be removed})}
% Experiments were performed to estimate evaporation of water from substrate. %(37.5x29.5x6~cm) 
% Two growing trays were filled with a mixture of 0.25~\si{\kilogram} substrate and 0.75~\si{\kilogram} water and then placed close to each other in the laboratory.
% A fan was placed next to one of the trays to blow a constant stream of air over the substrate.
% %The internal fan was activated with the lid left open to facilitate suitable conditions fr evaporation.
% The experiment was conducted over four days.
% Weight of each tray was measured up to twice every day.
% Laboratory temperature and humidity was constantly measured.
% Another similar experiment was performed, two trays were filled with a substrate mixture (1 dry feed: 3 water) and then placed close to each other in the laboratory.
% However, one tray had $50\%$ more surface area compared to the other.
% This experiment was conducted over four days and weight was measured up to three times per day.
% %It could be observed that evaporation from the tray with the fan was much faster than without.

\paragraph{Thermodynamics, heat and water fluxes}
Tests (TD1-TD6) were performed to identify the thermodynamic properties of the production unit and thus the energy and mass fluxes that takes place without any larvae and feed.
These experiments include: \begin{enumerate*}[label=(\arabic*)]
	\item passive cooling test without any growing medium, preheated chamber and allowed to dissipate the heat (TD1).
	\item Passive cooling test with growing medium filled with \SI{1}{\kilogram}water, covered with conductive film allowing only heat exchange (no water flux), preheated chamber and allowed to follow room temperature (TD2).
	\item automated heating-cooling test performed in an empty chamber to capture the dynamics of the heating-cooling TEC system (TD3).
	\item automated heating-cooling test performed growing medium filled with \SI{1}{\kilogram} water, covered with conductive film allowing only heat exchange to capture the convective heat transfer between the air and the growing medium (TD4).
	\item automated heating-cooling test performed with growing medium filled with \SI{1}{\kilogram} water, without any conductive film allowing both heat and water exchange to capture the convective heat transfer, evaporation and heat loss due to evaporation between the air and the growing medium (TD5).
	\item automated heating-cooling test performed with growing medium filled with \SI{1}{\kilogram} water, without any conductive film allowing both heat and water exchange and with ventilation (accelerated evaporation) to capture the convective heat transfer, evaporation rate and heat loss due to evaporation between the air and the growing medium (TD6).
\end{enumerate*}
In the automated heating-cooling tests, the TEC based heating-cooling system is set to +100\% and allowed to heat for \SI{1}{\hour} reaching temperature saturation.
The power is then reduced in steps of 5\% and allowed to saturate for \SI{20}{\minute} until the power reaches -100\% and then turned OFF to allow the temperatures to reach the outside temperatures passively.
This test covers a wide range of temperatures and direction for the heat and water fluxes.


 


==> symbol_list.tex <==
{
	\setlength{\LTleft}{-2.25in}
	\setlength{\LTright}{0in}
	\setlength{\LTcapwidth}{\dimexpr\textwidth+4.5in\relax}
	\begin{longtable}{@{\extracolsep{\fill}}lll@{}}
		\caption{\bf List of symbols used in the description of the models.} \label{tab:syms_list} \\ 
		\hline	\bf	Symbol                     & \bf Description                                		& \bf Unit                  \\ \hline \endfirsthead
		\caption[]{(continued ...)} \\
		\hline	\bf	Symbol                     & \bf Description                                		& \bf Unit                  \\ \hline 	\endhead
		\multicolumn{3}{r}{{continued on next page ...}} \\ \hline	\endfoot
		\hline \hline \endlastfoot
        $B_\mathrm{dry}$           & dry mass per larva 				        & [\si{\gram}]  \\
        $B_\mathrm{med}$           & combined mass of larvae, water and feed 				        & [\si{\kilogram}]  \\
        $B_\mathrm{wet}$           & wet mass per larva 				        & [\si{\gram}]  \\
        $B_\mathrm{tot}$           & total dry mass of all larvae in substrate  & [\si{\gram}]  \\
        $B_\mathrm{feed}$          & total feed available in the growing medium & [\si{\gram}]  \\
		$C_\mathrm{out}$           & CO$_2$ concentration of external source    		& [\si{\kilogram\per\meter\cubed}]  \\
		$C_\mathrm{air}$           & CO$_2$ concentration of air in production unit 	& [\si{\kilogram\per\meter\cubed}]  \\
		$H_\mathrm{air}$           & absolute humidity of the air in production unit    & [\si{\kilogram\per\meter\cubed}]  \\
		$H_\mathrm{out}$           & absolute humidity of external source       		& [\si{\kilogram\per\meter\cubed}]  \\
        $L_\mathrm{num}$           & total number of larvae surviving in the growing medium & [-]  \\
		$N_\mathrm{med}$           & feed present in medium          			& [\si{\kilogram}]               \\
		$N_\mathrm{exc}$           & larvae excreta present in medium          			& [\si{\kilogram}]               \\
		%$W_\mathrm{ovf}$           & total water overflowing                    & [\si{\kilogram}]               \\
        $T_\mathrm{air}$           & temperature of air in production unit          	& [\si{\celsius}]                \\
        $T_\mathrm{chm}$           & temperature on surface of inner chamber walls   & [\si{\celsius}]                \\
        $T_\mathrm{med}$           & temperature of growing medium in production unit   & [\si{\celsius}]                \\
		$T_\mathrm{hx}$            & temperature of the heat exchanger            		& [\si{\celsius}]                \\
        $T_\mathrm{out}$           & temperature of outside air                 		& [\si{\celsius}]                \\
		$T_\mathrm{\Sigma}$        & corrected temperature sums of larva       	& [\si{\celsius\hour}]                \\
        $O_\mathrm{air}$           & O$_2$ concentration of air in production unit 		& [\si{\kilogram\per\meter\cubed}]  \\
        $W_\mathrm{med}$           & total water in the growing medium          & [\si{\kilogram}]               \\
        $W_\mathrm{sto}$           & total water in the storage tank            & [\si{\kilogram}]               \\                
        $\phi_\mathrm{B_{assim}}$  & feed converted into energy and spent to digest the ingested feed  	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{B_{eff}}$  & effective assimilates available from the ingested feed for growth and maintenance 	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{B_{excr}}$ & flux of non digested feed back to substrate 	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{B_{ing}}$  & flux of feed from substrate into the larva 	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{B_{mat}}$  & assimilates spent towards building of new structure 	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{B_{maint}}$  & assimilates spent for maintenance of existing structure 	& [\si{\gram\per\second}]    \\
        $\phi_\mathrm{C_{bio}}$    & CO\textsubscript{2} production from biome & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{C_{exch}}$   & active exchange of CO\textsubscript{2} through pumps & [\si{\kilogram\per\second}] \\		
        $\phi_\mathrm{C_{leak}}$   & passive exchange of CO\textsubscript{2} through leakage & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{feed_{u}}$   & feed added to substrate as input & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{H_{chm}}$    & water vapor condensing on the inner walls of the production unit & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{H_{evap,med}}$   & evaporation from water surface & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{H_{exch}}$   & water vapor change due to air exchange during ventilation & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{H_{med}}$	   & net water movement between the growing medium and air (condensation and evaporation) & [\si{\kilogram\per\second}]\\
        $\phi_\mathrm{H_{u}}$	   & water vapor provided to or removed from the production unit through (de)humidifier & [\si{\kilogram\per\second}]\\
        $\phi_\mathrm{N_{assim}}$  & feed consumed by larvae & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{N_{biome}}$  & feed consumed by microbiome & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{N_{exc}}$  	& undigested feed excreted from larvae back into medium & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{O_{bio}}$    & O\textsubscript{2} consumption from biome & [\si{\kilogram\per\second}] \\
        $\phi_\mathrm{O_{exch}}$   & active exchange of O\textsubscript{2} through pumps & [\si{\kilogram\per\second}] \\		
        $\phi_\mathrm{O_{leak}}$   & passive exchange of O\textsubscript{2} through leakage & [\si{\kilogram\per\second}] \\		
        $\phi_{\mathrm{Q_{bio}}}$  & heat produced by the metabolic activities of the larvae and biome& [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{cond}}}$ & heat gained due to surface condensation of water& [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{evap}}}$ & heat lost from growing medium due to surface evaporation of water& [\si{\joule\per\second}]    \\
		$\phi_{\mathrm{Q_{exch}}}$ & heat exchanged with the outside through the ventilation/air circulation      & [\si{\joule\per\second}]    \\
		$\phi_{\mathrm{Q_{LED}}}$  & heat produced by LED lighting system         & [\si{\joule\per\second}]    \\
		$\phi_{\mathrm{Q_{L,chm}}}$& heat flux from evaporation and condensation of chamber walls  & [\si{\joule\per\second}]    \\
		$\phi_{\mathrm{Q_{L,med}}}$& heat flux from evaporation and condensation of substrate surface  & [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{loss}}}$ & heat conducted to the outside through the walls of the production unit       & [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{med}}}$  & heat transfered from the growing medium to the air through convection, radiation and conduction & [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{metab}}}$ & heat generated through larval metabolic activity& [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{rad}}}$  & heat lost through radiation from the growing medium to the surrounding& [\si{\joule\per\second}]    \\
        $\phi_{\mathrm{Q_{TEC}}}$  & heat produced/removed by heating/cooling system (TEC) of the production unit & [\si{\joule\per\second}]    \\
		$\phi_\mathrm{W_{bio}}$	   & water consumed by the larvae from the growing medium & [\si{\kilogram\per\second}]\\
		$\phi_\mathrm{W_{evap}}$   & water evaporation rate & [\si{\kilogram\per\second}]\\
		$\phi_\mathrm{W_{cond}}$   & water condensation rate & [\si{\kilogram\per\second}]\\
		$\phi_\mathrm{W_{cond,chm}}$  & condensation on chamber walls & [\si{\kilogram\per\second}] \\
		$\phi_\mathrm{W_{cond,TEC}}$  & condensation on TEC surface & [\si{\kilogram\per\second}] \\
		$\phi_\mathrm{W_{L,chm}}$  & evaporation and condensation from chamber walls & [\si{\kilogram\per\second}] \\
		$\phi_\mathrm{W_{L,TEC}}$  & evaporation and condensation from TEC surface & [\si{\kilogram\per\second}] \\
		$\phi_\mathrm{W_{L,med}}$  & evaporation and condensation from substrate surface & [\si{\kilogram\per\second}] \\
		$\phi_\mathrm{\dot{V}_u}$  & air exchange taking place through ventilator pumps      & [\si{\meter\cubed\per\second}] \\
        $\phi_\mathrm{W_{u}}$	   & water provided to the growing medium through pumps & [\si{\kilogram\per\second}]\\
		$k_\mathrm{a,q}$      	& Seebeck coefficient & [-] \\
        $k_\mathrm{A_{chm}}$ 		& total surface area of the production unit & [\si{\meter\squared}] \\
        $k_\mathrm{A_{half}}$  	& air flow rate for which the growth rate is reduced to half & [\si{\litre\per\minute}]  \\
        $k_\mathrm{A_{inf}A}$  	& infliction point for logistic model at which the growth rate is half for given airflow rate& [\si{\litre\per\minute\per\gram}]  \\
        $k_\mathrm{A_{med}}$ 		& top surface of the growing medium exposed to air							& [\si{\meter\squared}] \\
        $k_\mathrm{A_{medc}}$ 		& total surface area of growing medium container exposed to air				& [\si{\meter\squared}] \\
%        $k_\mathrm{A_{trans}}$  	& airflow rate influenced growth rate transition range for logistic model & [\si{\litre\per\minute\per\gram}]  \\		
		$k_\mathrm{B_{asy}}$  		& asymptotic size of the larvae in dry mass & [\si{\gram}]    \\
        $k_\mathrm{B_{half}gm}$ & feed density/feeding rate for which the development rate is half & [\si{\gram\per\gram\per\day}]   \\
        $k_\mathrm{bio_{C}}$ & specific rate of CO$_2$ production from metabolic activity of microbiome & [\si{\gram\per\gram}] \\
        $k_\mathrm{bio_{Q}}$ & specific rate of heat production from metabolic activity of microbiome & [\si{\watt\per\gram}] \\
        $k_\mathrm{bio_{O}}$ & specific rate of O$_2$ consumption from metabolic activity of microbiome & [\si{\gram\per\gram}] \\
		$k_\mathrm{c_{air}}$ 		& specific heat capacity of air             & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{C_{chm}}$ 		& specific heat capacity of complete growing chamber           & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{C_{med}}$ 		& specific heat capacity of complete growing tray           & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{C:O}$			& ratio of O\textsubscript{2} consumed to CO\textsubscript{2} produced    & [-] \\
		$k_\mathrm{c_{vap}}$		& specific heat capacity of water vapor    & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{c_{chm}}$		& specific heat capacity of chamber internal parts  & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{c_{feed}}$		& specific heat capacity of feed (dry mass)     & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{c_{tray}}$		& specific heat capacity of growing tray     		& [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{c_{water}}$		& specific heat capacity of water     		& [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{c_{lrv}}$		& specific heat capacity of larvae biomass  & [\si{\joule\per\kelvin\per\kilogram}] \\
		$k_\mathrm{dev_{ts}}$  		& conversion factor to obtain development sum in hours & [\si{\per\second}]   \\
        $k_{\mathrm{heat}i}$		& heat dissipated by LED channel number $i$ & [-] \\
        $k_\mathrm{h_{chm}}$ 		& heat transfer coefficient of between air and walls of the production unit (conduction) 	& [\si{\watt\per\meter\squared\per\kelvin}] \\
        $k_\mathrm{h_{ew}}$			& latent heat of vaporization of water			& [\si{\kilo\joule\per\kilogram}] \\
        $k_\mathrm{h_{med}}$ 		& heat transfer coefficient of air (convection)	& [\si{\watt\per\meter\squared\per\kelvin}] \\
        $k_\mathrm{inges}$ 		& specific ingestion rate of larva & [\si{\gram\per\gram\second}] \\
        $k_\mathrm{Le}$ & lewis number & [-] \\
        $k_\mathrm{lrv_{Q}}$ & specific rate of heat production from metabolic activity of larvae & [\si{\watt\per\gram}] \\
        $k_\mathrm{lrv_{C}}$ & specific rate of CO$_2$ production from metabolic activity of larvae & [\si{\gram\per\gram}] \\
        $k_\mathrm{lrv_{O}}$ & specific rate of O$_2$ consumption from metabolic activities of larvae & [\si{\gram\per\gram}] \\
        $k_\mathrm{maint}$ 		& specific rate of maintenance and maturity of larva & [\si{\gram\per\gram\per\second}] \\
        $k_\mathrm{Q_{cond}}$ 		& fraction of heat lost to the outer surface & [-] \\
        $k_\mathrm{r_{base}T}$  & minimum development rate observed above the lower temperature boundary (Logan-10 model) & [\si{\per\second}]   \\
        $k_\mathrm{R_g}$	& gas constant & [\si{\joule\per\kelvin\per\mole}] \\
        $k_\mathrm{R,q}$			& series resistance TEC & [-] \\
        $k_\mathrm{r_{max}A}$  	& maximum observed growth rate in response to airflow rate & [\si{\gram\per\second}]  \\
        $k_\mathrm{r_{max}dm}$  	& maximum development rate of the larvae in response to feed density/availability & [\si{\per\second}]   \\
        $k_\mathrm{r_{max}gm}$  	& maximum growth rate of the larvae in response to feed density/availability & [\si{\gram\per\second}]   \\
        $k_\mathrm{r_{max}T}$  	& maximum observed development rate in response to temperature (Logan-10 model) & [\si{\per\second}]   \\
        $k_\mathrm{r_{max}W}$   & maximum growth rate in response to feed moisture concentration & [\si{\gram\per\day}]\\
        $k_\mathrm{r_{ref}T}$ & development rate observed at the known reference temperature $k_\mathrm{T_{ref}}$ & [\si{\per\second}]    \\
        $k_\mathrm{\rho T}$  & development rate change per degree change in temperature (Logan-10 model) & [\si{\per\celsius}]   \\
        $k_\mathrm{T_{base}}$   & lower temperature boundary above which the development is observed (Logan-10 model)& [\si{\celsius}]   \\
        $k_\mathrm{T_{max}}$  	& lethal maximum temperature for larval survival (modified Logan-10 model)& [\si{\celsius}]   \\
        $k_\mathrm{T_{ref}}$			& reference temperature for Magnus-Tetens equation & [\si\kelvin] \\
        $k_\mathrm{T_{\Sigma}1}$  	& development point at which the assimilation process starts to cease & [\si{\hour}]   \\
        $k_\mathrm{T_{\Sigma}2}$  	& development point at which the assimilation process ends & [\si{\hour}]   \\
        $k_\mathrm{T_{\Sigma}3}$  	& development point at which the larval development phase ends & [\si{\hour}]   \\
        $k_\mathrm{TEC}$			& thermal conductivity TEC & [-] \\
        $k_\mathrm{U_{chm}}$ 		& heat transfer coefficient of walls of the production unit (conduction) 	& [\si{\watt\per\meter\squared\per\kelvin}] \\
        $k_\mathrm{V_{chm}}$ 		& total volume inside the production unit 		& [\si{\meter\cubed}] \\
        $k_\mathrm{\dot{V}_{leak}}$ & gas leakage rate in the production unit & [\si{\meter\cubed\per\second}] \\
        $k_\mathrm{w_{assim}}$      & fraction of water consumed by larvae for every gram of feed assimilated & [-] \\
        $k_\mathrm{W_{med}C1}$ & lowest feed moisture below which the growth ceases & [\si{\gram\per\gram}]   \\
        $k_\mathrm{W_{med}C2}$ & feed moisture above which the ingestion rate can reach maximum & [\si{\gram\per\gram}]   \\
        $k_\mathrm{W_{med}C3}$ & feed moisture above which the diffusion of oxygen/air exchange starts to cease & [\si{\gram\per\gram}]   \\
        $k_\mathrm{W_{med}crit}$ & feed moisture  above which the larvae begins to die & [\si{\gram\per\gram}]   \\
        $k_\mathrm{W_{mmol}}$	& molar mass of water & [\si{\gram\per\mole}] \\
        $k_\mathrm{W_{per}}$		& minimum moisture concentration for maximum evaporation & [-] \\
		$k_\mathrm{\Delta T}$  	& width of the high temperature boundary (modified Logan-10 model)& [\si{\celsius}]   \\
		$k_\mathrm{\epsilon_{dry}}$	& correction factor for evaporation coefficient & [-] \\
        $k_\mathrm{\epsilon_{inges}}$ 	& conversion efficiency of feed ingestion & [-] \\
		$k_\mathrm{\epsilon_{med}}$ 		& emissivity of growing medium surface	& [\si{\watt\per\meter\squared\per\kelvin}] \\
        $k_\mathrm{\rho_{air}}$ 	& density of air             				& [\si{\kilogram\per\meter\cubed}] \\
		$k_\mathrm{\sigma_{rad}}$ 	& Stefan-Boltzmann Constant						& [\si{\watt\per\meter\squared\kelvin}$^{-4}$] \\

		$r_\mathrm{assim}$ 		& regulation of assimilation rate in response to internal and external factors & [-] \\
		$r_\mathrm{mat}$ 		& regulation of maturity-maintenance rate in response to internal and external factors & [-] \\
        $rc_\mathrm{A}$  	& normalized larva growth rate in response to air flow rate & [\si{\gram\per\second}]    \\
        $rc_\mathrm{F}$  	& normalized larva development rate in response to feed density & [\si{\per\second}]    \\
        $rc_\mathrm{F_{grw}}$  	& normalized larva growth rate in response to feed density & [\si{\gram\per\second}]    \\
		$rc_\mathrm{T}$  	& normalized larva development rate in response to substrate temperature & [\si{\per\second}]    \\
		$rc_\mathrm{W}$  	& normalized larva growth rate in response to substrate moisture & [\si{\gram\per\second}]    \\
		$V_\mathrm{max}$ 		& maximum applicable voltage to TEC & [-] \\
        $\epsilon_\mathrm{evap}$ 		& efficiency of evaporation as function of water content & [-] \\
        $\epsilon_\mathrm{inges}$ 		& efficiency of the ingested feed & [-] \\
%		\multicolumn{3}{c}{{\red{needs to be updated}}} \\
	\end{longtable}
	%\begin{flushleft} Table notes Phasellus venenatis, tortor nec vestibulum mattis, massa tortor interdum felis, nec pellentesque metus tortor nec nisl. Ut ornare mauris tellus, vel dapibus arcu suscipit sed.
	%\end{flushleft}
}

